Tuning Streamed Applications on Intel Xeon Phi: A Machine Learning Based Approach

Many-core accelerators, as represented by the XeonPhi coprocessors and GPGPUs, allow software to exploit spatial and temporal sharing of computing resources to improve the overall system performance. To unlock this performance potential requires software to effectively partition the hardware resource to maximize the overlap between hostdevice communication and accelerator computation, and to match the granularity of task parallelism to the resource partition. However, determining the right resource partition and task parallelism on a per program, per dataset basis is challenging. This is because the number of possible solutions is huge, and the benefit of choosing the right solution may be large, but mistakes can seriously hurt the performance. In this paper, we present an automatic approach to determine the hardware resource partition and the task granularity for any given application, targeting the Intel XeonPhi architecture. Instead of hand-crafting the heuristic for which the process will have to repeat for each hardware generation, we employ machine learning techniques to automatically learn it. We achieve this by first learning a predictive model offline using training programs; we then use the learned model to predict the resource partition and task granularity for any unseen programs at runtime. We apply our approach to 23 representative parallel applications and evaluate it on a CPU-XeonPhi mixed heterogenous many-core platform. Our approach achieves, on average, a 1.6x (upto 5.6x) speedup, which translates to 94.5% of the performance delivered by a theoretically perfect predictor.

==> data/speedup_over_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'dct'
%\begin{table*}[htbp]
%  \centering
%  \scriptsize
%  \caption{Speedup of dataset-configuration pairs}
%    \begin{tabular}{lrrrrrrrrrrrrrrrr}
%\toprule
%    \multirow{2}[0]{*}{Config.} & \multicolumn{16}{c}{Dataset} \\\cmidrule(r){2-17}
%          & \multicolumn{1}{l}{8M} & \multicolumn{1}{l}{16M} & \multicolumn{1}{l}{24M} & \multicolumn{1}{l}{32M} & \multicolumn{1}{l}{40M} & \multicolumn{1}{l}{48M} & \multicolumn{1}{l}{56M} & \multicolumn{1}{l}{64M} & \multicolumn{1}{l}{72M} & \multicolumn{1}{l}{80M} & \multicolumn{1}{l}{88M} & \multicolumn{1}{l}{96M} & \multicolumn{1}{l}{104M} & \multicolumn{1}{l}{112M} & \multicolumn{1}{l}{120M} & \multicolumn{1}{l}{128M} \\
%\midrule
%    (40,80) & \textbf{1.41} & 1.33  & 1.10  & 1.17  & 1.16  & 1.15  & 1.07  & 1.07  & 1.01  & 0.86  & 0.98  & 0.96  & 1.04  & 1.05  & 0.86  & 0.99  \\
%    (36,108) & 1.28  & \textbf{1.46} & 1.27  & 1.17  & 1.18  & 1.09  & 1.14  & 1.05  & 1.00  & 0.97  & 1.05  & 1.00  & 1.05  & 0.98  & 1.01  & 0.75  \\
%    (29,116) & 1.28  & 1.18  & \textbf{1.29} & 1.22  & 1.14  & 1.00  & 1.05  & 1.00  & 1.04  & 0.95  & 1.03  & 0.96  & 0.99  & 1.01  & 0.99  & 1.03  \\
%    (9,54) & 1.14  & 1.06  & 1.05  & \textbf{1.33} & 1.23  & 1.19  & 1.14  & 1.12  & 1.16  & 1.11  & 1.06  & 1.00  & 0.98  & 0.46  & 1.06  & 0.85  \\
%    (11,66) & 1.16  & 1.15  & 1.20  & 1.12  & \textbf{1.27} & 1.18  & 1.15  & 1.13  & 1.08  & 1.08  & 1.00  & 0.98  & 0.96  & 0.99  & 1.06  & 1.03  \\
%    (16,80) & 1.24  & 1.06  & 1.08  & 1.16  & 1.19  & \textbf{1.24} & 1.20  & 1.06  & 1.11  & 0.96  & 0.94  & 0.94  & 1.06  & 0.93  & 1.02  & 1.06  \\
%    (20,100) & 1.16  & 1.10  & 1.13  & 1.21  & 1.20  & 1.10  & \textbf{1.31} & 1.09  & 1.13  & 0.97  & 0.99  & 0.95  & 0.99  & 0.56  & 0.95  & 1.03  \\
%    (17,85) & 1.23  & 1.05  & 1.21  & 1.15  & 1.12  & 1.14  & 1.17  & \textbf{1.14} & 1.14  & 0.90  & 0.98  & 1.05  & 0.99  & 0.43  & 0.99  & 1.02  \\
%    (16,80) & 1.19  & 1.07  & 1.10  & 1.17  & 1.22  & 1.21  & 1.20  & 1.11  & \textbf{1.17} & 0.99  & 1.04  & 0.96  & 1.00  & 0.63  & 0.97  & 1.06  \\
%    (13,78) & 1.13  & 0.97  & 1.07  & 1.05  & 1.27  & 1.14  & 1.24  & 0.98  & 1.04  & \textbf{1.15} & 0.94  & 1.03  & 0.96  & 0.41  & 0.99  & 1.00  \\
%    (27,162) & 1.15  & 1.13  & 1.08  & 1.19  & 1.10  & 1.08  & 1.15  & 0.97  & 0.97  & 1.01  & \textbf{1.11} & 0.80  & 1.02  & 0.96  & 1.02  & 1.00  \\
%    (11,77) & 1.02  & 0.94  & 1.17  & 1.17  & 1.21  & 1.10  & 1.17  & 0.94  & 1.00  & 0.96  & 0.96  & \textbf{1.06} & 1.04  & 0.47  & 1.08  & 1.10  \\
%    (16,128) & 0.94  & 0.96  & 0.96  & 1.22  & 0.96  & 1.05  & 1.00  & 0.86  & 0.95  & 0.95  & 1.00  & 1.04  & \textbf{1.17} & 0.49  & 0.98  & 0.99  \\
%    (19,190) & 0.89  & 1.03  & 0.81  & 0.89  & 0.89  & 0.86  & 0.84  & 0.91  & 0.92  & 1.04  & 0.92  & 0.99  & 1.00  & \textbf{1.07} & 1.04  & 1.10  \\
%    (23,207) & 1.01  & 1.10  & 1.08  & 1.11  & 1.05  & 1.01  & 0.98  & 0.88  & 0.88  & 0.90  & 0.95  & 0.95  & 1.04  & 0.95  & \textbf{1.11} & 0.96  \\
%    (12,108) & 0.82  & 0.81  & 0.97  & 1.12  & 1.02  & 1.07  & 1.00  & 0.94  & 0.96  & 0.99  & 1.06  & 1.02  & 1.04  & 0.41  & 1.03  & \textbf{1.14} \\
%\bottomrule
%    \end{tabular}%
%  \label{tab:speedup_od}%
%\vspace{-5mm}
%\end{table*}%


\begin{figure*}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.8]{heatmap_dataset.pdf}\\
  \caption{Performance of best-performing configurations across input datasets for \texttt{dct}. The best streamed configuration varies across inputs and a good configuration on one input
  can give poor performance on another dataset.}\label{}
\end{figure*}


==> lst/source_out.tex <==
__kernel void A(__global char* a, short b, int c) {
  const int d = get_global_id(0);
  a[d] = b;
}

==> mlstream_features.tex <==
\section{Extracting Features} 
\subsection{Program Features}
We use four categories of features to represent programs: \texttt{kernel features}, \texttt{transfer features}, \texttt{task features}, and \texttt{dynamic features}. 

The \texttt{kernel features} relate to the kernel loops and their parallelization. The first kernel feature is on \texttt{data types}. The transferred data can be stored on the coprocessor's memory in different data types such as \textit{integer}, \textit{float}, etc. Correspondingly, the kernel will use different ALUs. The second kernel feature is on the parallelization candidate--\texttt{parallelization location} and \texttt{loop counts}. With the \texttt{omp clause}, we can parallelize the kernel at either the outer loop or the inner loop. Besides, \texttt{loop counts} reflects the total amount of work. These features can be obtained from the kernel source code. 

The \texttt{transfer features} are the features on data transfers between the host CPU and the coprocessor. \texttt{xfer\_mem count} is referred to as the number of occurrence of the data transfer API, and indicates the number of data structures which are moved between host and coprocessor. This feature can be derived from the source code. The second transfer feature is \texttt{redundant transfers}. That is, the data regions required by contiguous tasks are partially overlapped. Thus, we have to transfer redundant data elements (i.e., ghost region) for each task. This feature is application-dependent: some applications are embarrassingly parallel while others are false-dependent~\cite{DBLP:journals/ppl/FangZLTCCY16}. We can obtain this feature by calculating the area of the ghost region. The third transfer-related feature is on the amount of moved data, i.e., \texttt{transferred data amount}. This feature can be calculated by knowing the size of input datasets.

Another category of features are related to tasks. The first task feature is \texttt{maximum blocks} which denotes the maximum number of tasks for a given application and input dataset. This feature indicates the maximum number of concurrent tasks running in the pipeline. On the other hand, we use \texttt{minimum task unit} to represent the minimum task unit. This feature indicates the minimum task unit running on a partition. 

Beside the static code features, we use dynamic kernel features including \texttt{instructions}, \texttt{branch miss}, and \texttt{L1 data cache miss}. The features reflect how code behaves on the computing units. The values are obtained by profiling the non-streamed kernels with \texttt{Intel's VTune}. 

\subsection{Merging Labels}

